Time-to-Label: Temporal Consistency for Self-Supervised Monocular 3D Object Detection

Monocular 3D object detection continues to attract attention due to the cost benefits and wider availability of RGB cameras. Despite the recent advances and the ability to acquire data at scale, annotation cost and complexity still limit the size of 3D object detection datasets in the supervised settings. Self-supervised methods, on the other hand, aim at training deep networks relying on pretext tasks or various consistency constraints. Moreover, other 3D perception tasks (such as depth estimation) have shown the benefits of temporal priors as a self-supervision signal. In this work, we argue that the temporal consistency on the level of object poses, provides an important supervision signal given the strong prior on physical motion. Specifically, we propose a self-supervised loss which uses this consistency, in addition to render-and-compare losses, to refine noisy pose predictions and derive high-quality pseudo labels. To assess the effectiveness of the proposed method, we finetune a synthetically trained monocular 3D object detection model using the pseudo-labels that we generated on real data. Evaluation on the standard KITTI3D benchmark demonstrates that our method reaches competitive performance compared to other monocular self-supervised and supervised methods.

==> sections/analysis.tex <==
\section{Analysis}
\begin{comment}
\subsection{Temporal coherence in KITTI}
\label{kitti_temporal_coherence}
Using temporal prior present in videos to simplify per-frame tasks is a long-standing idea. Applying this prior in the context of object detection tasks in the presence of camera motion, however, requires access to accurate pose measurements and assumes that object annotations are coherent across time.
In practice, ego-pose information is used to construct a global reference system. In this step sensor noise and drift may accumulate an error in the map projection, and thus in localization. Additionally, temporally coherent labels are more challenging to obtain. According to KITTI \cite{kitti}, for example, the annotation process was carried out on each frame independently. To address these issues, and to quantitatively assess the incoherence of the temporal propagation in KITTI, we carry out the following experiment. First, we consider the ground truth of KITTI training set, in which we identify static objects, by projecting cars positions from the local to the global reference system and applying a simple heuristic of 2.5 meters threshold. Ideally, we would expect different observations of the same static object to project in the same map point. In Figure \ref{fig:ranges}, we plot the range of obtained map projections for the static objects, which shows that most of the static objects ( $\approx$ 75\%) are indeed projected to the global map with less than 0.5 meters drift on the three axes. The remaining 25\% , on the other hand, exhibit a larger variation, with some outliers suffering from drastic drifts. 
\begin{figure}
\center
      \includegraphics[height=4cm]{Figures/rangesmap.png}
      
      \caption{Position ranges for static objects when projected to the global reference system. X,Y,Z are the axes in the IMU reference system}
      \label{fig:ranges}
  \end{figure}

To quantify the effect of this drift on the benchmark, we first calculate a single map position for each of the static objects by simply averaging the frame-wise observations projected on the map. Next, we back-project this location to each frame, using the ego-motion known transformations, while keeping all other properties (2D box, rotation, size ,..) without modification. Finally, we evaluate this temporally consistent version of the ground truth against the original one, using KITTI official benchmark. Ideally, if KITTI labels were consistent with the ego-motion transformations, we would expect the AP benchmark to yield 100\% accuracy. Table \ref{table:gt_temporal_drift}, however, shows a degraded AP (both in 3D and in BEV) across different IoU thresholds. Results  suggest that the 3D localization of objects suffer with temporal coherence, while Bird's eye view results shows only a minor degradation, possibly indicating a significant impact of the pitch angle of the ego vehicle.
\begin{table}[h!]
\centering
\small
\begin{tabular}{c|*3c|*3c}
 \midrule
  & \multicolumn{3}{c}{AP 3D \%} & \multicolumn{3}{c}{AP BEV \%}\\
 \midrule
&Easy&Mod&Hard&Easy&Mod&Hard\\ 
\midrule\midrule
IoU@0.5 & 83.73&84.24&84.24&94.79&95.30&95.33\\
\midrule
IoU@0.7 & 48.55&45.68&45.68&79.41&79.67&79.69\\
\midrule\midrule
\end{tabular}
\caption{Evaluation of ground truth when enforcing temporal coherence using the ego-motion measurements}


\label{table:gt_temporal_drift}
\end{table}

\end{comment}
\begin{comment}
\subsection{Tracking Performance}
Since we rely on object trajectories to infer a temporal evolution and motion state of objects, it is important to build consistent object trajectories using tracking and association. While outside the scope of this work, shape prior and the detector itself can be used to extract appearance or geometric cues to associate objects. Relying only on the external 3D tracker \cite{baseline_tracker}, the main factor controlling the tracking accuracy are the detections themselves (in 3D). One way to assess this accuracy is to use the 2D tracking benchmark available in KITTI. It is worth mentioning that our 2D detection accuracy is not on par with other 2D detectors trained on KITTI, since we do not finetune the synthetic model on any real KITTI labels, but it is, nevertheless, useful to note the positive trend of the 2D detection across subsequent finetuning stages, and consequently, the tracking performance measured in terms of Identification F1 score (IDF1) \cite{idf1}.
Table \ref{table:dettrack} reports the 2D detection and tracking benchmark evaluated for different iterations of pseudo-labels from the KITTI train split \cite{split} using the KITTI evaluation code \cite{tracking_code}
\begin{table}[h!]
\centering
\small
\begin{tabular}{*8c}
 \hline
  &\multicolumn{3}{c}{AP 2D \%} & \\
 \hline\hline
Iteration&Easy&Mod&Hard&IDF1\\ 
1st&84.46&63.21&56.02&41.51\\
2nd&91.52&67.31&57.65&51.94\\
3rd&91.91&69.78&60.10&56.24\\
\hline

\end{tabular}
\caption{2D Detection and Tracking performance measured in the three pseudo-label iterations on KITTI trainsplit and using the official benchmark}


\label{table:dettrack}
\end{table}
\end{comment}
